A Quantum Algorithm for Finding $k$-Minima

We propose a new finding $k$-minima algorithm and prove that its query complexity is $\mathcal{O}(\sqrt{kN})$, where $N$ is the number of data indices. Though the complexity is equivalent to that of an existing method, the proposed is simpler. The main idea of the proposed algorithm is to search a good threshold that is near the $k$-th smallest data. Then, by using the generalization of amplitude amplification, all $k$ data are found out of order and the query complexity is $\mathcal{O}(\sqrt{kN})$. This generalization of amplitude amplification is also not well discussed and we briefly prove the query complexity. Our algorithm can be directly adapted to distance-related problems like $k$-nearest neighbor search and clustering and classification. There are few quantum algorithms that return multiple answers and they are not well discussed.

==> abst.tex <==
We propose an algorithm that finds $k$ minima. 
This algorithm finds the number of $k$ indices that have minimum value from an unsorted table of $N$ items.
Our algorithm's computational complexity is $\mathcal{O}(\sqrt{kN})$.
This is 

